A Human-Grounded Evaluation Benchmark for Local Explanations of Machine Learning

Research in interpretable machine learning proposes different computational and human subject approaches to evaluate model saliency explanations. These approaches measure different qualities of explanations to achieve diverse goals in designing interpretable machine learning systems. In this paper, we propose a human attention benchmark for image and text domains using multi-layer human attention masks aggregated from multiple human annotators. We then present an evaluation study to evaluate model saliency explanations obtained using Grad-cam and LIME techniques. We demonstrate our benchmark's utility for quantitative evaluation of model explanations by comparing it with human subjective ratings and ground-truth single-layer segmentation masks evaluations. Our study results show that our threshold agnostic evaluation method with the human attention baseline is more effective than single-layer object segmentation masks to ground truth. Our experiments also reveal user biases in the subjective rating of model saliency explanations.

==> files/old-stuff.tex <==







% \section{Evaluation Benchmark}

In order to create a human-grounded benchmark for model explanations evaluation, we captured human annotation of salient features where participants were asked to select relevant regions in images and phrases in text documents that are representing the topic or subject.
The preliminary deployment of this benchmark consists of a subset of 100 sample images and text articles from the well-known \textit{ImageNet} \cite{deng2009imagenet} and \textit{20 Newsgroup} \cite{Lang95newwgroup} data sets. 



\noindent \textit{Annotated Image Samples:}

All image samples were collected from the \textit{ImageNet} data set from 20 general categories (example categories include animals, plants, humans, indoor objects, and outdoor objects). 
Our preliminary benchmark includes 5 images per category for a total of 100 images. 
In an IRB approved participation study, 10 participants viewed images on a tablet and used a stylus to annotate key regions of the image.
We asked them to draw a contour in the image around the area most important to recognize the object or the portion that, if removed, you could not recognize the object. 
None of the participants were experts in any of the image categories.
Each participant annotated all images in a random ordering. 

All participants' annotations are accumulated to create a weighted explanation mask over the image. 
Figure~\ref{fig:userheatmaps}-a shows a heatmap view of participants' annotated explanations over a sample image, where ``hot'' colors (red) shows more commonly highlighted regions, and ``cooler'' colors (blue) show areas that were highlighted less frequently. 
We also masked all participants' annotations with exact contour shapes to reduce the impact of participants' imprecision or hand jitter. 
% As described before, users different opinion on explanations results in weighted salient features in the image. 


\noindent \textit{Annotated Text Samples:} All text documents were collected from the \textit{20 Newsgroup} data set in medical (\textit{sci.med}) and electronic (\textit{sci.elect}) categories.
For each category, two expert reviewers highlighted the most important words relevant to the given topic (i.e., medical or electronic). 
Reviewers were instructed to highlight words which, if removed, you could not recognize the main topic of the article. 
Two electrical engineers and two physicians volunteered as experts to annotate 100 documents from each topic.
Each expert annotated the documents individually and in random order. 
Figure~\ref{fig:userheatmaps}-b shows a single tone heat map view of user annotated explanations over a partial sample text article. 




\begin{figure}[t!]
\centering
  \includegraphics[width=1.0\columnwidth]{figures/catmask.jpg}
  (a)
  \includegraphics[width=1.0\columnwidth]{figures/catlime2.png}
  (b)
  \caption{(a) User generated weighted-mask for an example from ImageNet. We use this weighted-mask to evaluate model explanations accuracy. 
    (b) Model explanation using LIME~[8] algorithm for the same image.
    Irrelevant red-highlighted regions in this image cause low explanation score in comparison to the human-grounded annotation.}
  \label{fig:usermask}
\end{figure}



==> files/old_3.2-procedure.tex <==
%%%%%%%%%%%%
%%not being imported right now
%%%%%%%%%%%%


% \subsection{Annotation Procedure:} 
% \sina{need a sentence or two about the data set used in our study:}

% In an IRB approved participation study, we asked \sina{#participants} Amazon Mechanical Turkers to complete the annotation task.
% A tutorial was provided to Turkers in order to introduce the interface with a series of screenshots and short captions. 
% As a control, each screenshot and caption was displayed on screen for 2 seconds before participants were able to continue to the next slide.
% Participants were told they were helping choose the ``image areas that best represent items'' or ``most descriptive words'' to train our AI system.

% % Since our participants come from Amazon Mechanical Turk, we assume that none of the participants were experts in any of the image or textual categories.
% Each participant annotated 14 images or documents in a systematic way to ensure there was enough random variability in how participants were annotating each classification.
% Each image or document was annotated by 10 different participants and the accumulated annotations create the  weighted explanation mask seen in Figure \ref{fig:userheatmaps}.
% For text annotations, \sina{What did we do to reduce variability?}
% For image annotations, We also masked all participants' annotations with an exact contour shape to reduce the impact of participants' imprecision or hand jitter. 


% For each category, expert reviewers highlighted the most important words relevant to the given topic name (i.e., medical or electronic).
% Domain experts reviewers were instructed to highlight words which, if removed, you could not recognize the main topic of the article. 
% Two electrical engineers and two physicians volunteered as experts to annotate 100 documents from each topic.



==> files/old_4.3-experiments_3.tex <==
%%%%%%%%%%%%
%%not being imported right now
%%%%%%%%%%%%





% \subsubsection{User Biases in Model Error}
% We explored human judgment evaluation results to find other possible external or internal factors that could affect participants' subjective ratings. 
% Examples include participants' prior-knowledge and expectations that could interfere their ratings. 
% We reviewed results to identify possible participants' biases toward model explanation FP and FN error types. 


% To analyze participants' rating behavior in different error types, we first divided in two groups of examples with high FP explanation error and high FN explanation errors. 
% We then reviewed participants' rating between two groups. 
% Two regression 
% This indicates that users pay less attention to FP errors (when model is looking at background pixels) and in turn are more critical when model is missing at foreground pixels.


% \begin{figure}[t!]
% \centering
% \begin{subfigure}[b]{0.49\columnwidth}
%         \includegraphics[width=1.0\columnwidth]{figures/user-bias.PNG}
%         \caption{(a)}
%     \end{subfigure}
%       \hfill
%     \begin{subfigure}[b]{0.49\columnwidth}
%         \includegraphics[width=1.0\columnwidth]{figures/user-bias-2.PNG}
%         \caption{(b)}
%     \end{subfigure}
%   \caption{(a) .... (b) ....}
%   \label{fig:results-2}
% \end{figure}



==> files/proxy_old-2.1._.tex <==
% -- this part is out --

\subsection{Proxy Evaluation of Explanations}
% \subsection{Task-Grounded Evaluation of XAI} 
% \subsection{Proxy Evaluation of XAI}

A line of research on XAI evaluation methods, studies effects of machine learning explanations on end-users in different setup. 
Mohseni et al.~\cite{mohseni2019survey} reviews different measures used to evaluate XAI systems including: 1) task performance, 2) trust and reliance, and 3) preference and engagement. 
Also, various subjective and objective metrics have been proposed for these measurements. 
For example, subjective ratings such as user perceived understanding~\cite{papenmeier2019model}, as well as objective measures for user agreement rate with AI suggestion~\cite{yin2019understanding} are used for trust and reliance evaluation. 
Plus, participants' success rate and task duration are from common task performance metrics~\TODO{cite}. 
However, there are certain limitations in results implications and interpretations for explanations evaluation through a task proxy. 
First, human-AI collaboration tasks are greatly influenced by the choice of user task complexity, user familiarity with the task,  and data complexity. 
Two studies on effects of model explanations on task performance in \TODO{x et al.} and \TODO{y et al.} papers present somewhat counter results. 
Therefore, different papers in this area present different results. 
Second, different subjective and objective measures for user behavior do not necessary align which causes interpretation ambiguity.
For example, ... \TODO{cite}.


Moreover, there exists inevitable human factors in proxy studies that, in some cases, it seems impractical to run legitimate accurate controlled study.
For example, Buccinca et al.~\cite{buccinca2020proxy} present experiments on a food recommendation case study in which shows objective task performance measures do not correlate with subjective measures of user preference, trust, and user prediction of model output. 
Authors also review the impact of think-aloud method on participants behavior in their qualitative study. 
Another example in proxy evaluation is the impact of placebic explanations on user trust\cite{langer1978mindlessness}.
In a recent work, Eiband et al.~\cite{eiband2019impact} observed placebic explanations improve user trust on AI recommendations.
They suggest using placebic explanations as the baseline condition instead of non-explainable AI as a baseline in studying user reliance and performance on XAI systems. 
Therefore, this question remains that whether proxy evaluation of model explanations with different tasks and conditions is a reliable approach for this goal.



